Field of View Extension in Computed Tomography Using Deep Learning Prior

In computed tomography (CT), data truncation is a common problem. Images reconstructed by the standard filtered back-projection algorithm from truncated data suffer from cupping artifacts inside the field-of-view (FOV), while anatomical structures are severely distorted or missing outside the FOV. Deep learning, particularly the U-Net, has been applied to extend the FOV as a post-processing method. Since image-to-image prediction neglects the data fidelity to measured projection data, incorrect structures, even inside the FOV, might be reconstructed by such an approach. Therefore, generating reconstructed images directly from a post-processing neural network is inadequate. In this work, we propose a data consistent reconstruction method, which utilizes deep learning reconstruction as prior for extrapolating truncated projections and a conventional iterative reconstruction to constrain the reconstruction consistent to measured raw data. Its efficacy is demonstrated in our study, achieving small average root-mean-square error of 24 HU inside the FOV and a high structure similarity index of 0.993 for the whole body area on a test patient's CT data.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% Horsch 041224
%
% - übernommen von Lehmann
% - angepasst für Proceedings BVM2003, Erlangen, Jan 2003
%	- Pseudo-Definitionen für tocgenerate (Generierung Inhaltsverz.)
%   \pagecount (Dez 2004)
%

\catcode`@=11

\def\makeauthor{\if@filesw \newwrite\@aindexfile
  \immediate\openout\@aindexfile=\jobname_authors.pix
  \def\addauthor{\@bsphack\begingroup
             \def\protect####1{\string####1\space}\@sanitize
             \@wraindex}\typeout
  {Writing index file \jobname_authors.pix }\fi}

\def\@wraindex#1{
   \edef\@tempa{\write\@aindexfile{{#1}{\the\tocpos}}}
        \expandafter\endgroup\@tempa
   \if@nobreak \ifvmode\nobreak\fi\fi\@esphack}

\def\addauthor{\@bsphack\begingroup \@sanitize\@addauthor}

\def\makepreindex{\if@filesw \newwrite\@pindexfile
  \immediate\openout\@pindexfile=\jobname_index.pix
  \def\addpreindex{\@bsphack\begingroup
             \def\protect####1{\string####1\space}\@sanitize
             \@wrpindex}\typeout
  {Writing index file \jobname_authors.pix }\fi}

\def\@wrpindex#1{
   \edef\@tempa{\write\@pindexfile{{#1}{\the\tocpos}}}
        \expandafter\endgroup\@tempa
   \if@nobreak \ifvmode\nobreak\fi\fi\@esphack}

\def\addpreindex{\@bsphack\begingroup \@sanitize\@addpreindex}

\def\makecategory{\if@filesw \newwrite\@bindexfile
  \immediate\openout\@bindexfile=\jobname_category.pix
  \def\addcategory{\@bsphack\begingroup
             \def\protect####1{\string####1\space}\@sanitize
             \@wrbindex}\typeout
  {Writing index file \jobname_category.pix }\fi}

\def\@wrbindex#1{
   \edef\@tempa{\write\@bindexfile{{#1}{\the\tocpos}}}
        \expandafter\endgroup\@tempa
   \if@nobreak \ifvmode\nobreak\fi\fi\@esphack}

\def\addcategory{\@bsphack\begingroup \@sanitize\@addcategory}

\catcode`@=12




% \newcommand{\tocentry}[7]
\newcommand{\tocentry}[5]
% #1 = articletype + counter
% #2 = title
% #3 = Autoren
% #4 = Autoren, erster fett
% #5 = Seitenzahl
           {
            %\vspace{3mm}
            \noindent
%ho            \begin{minipage}[b]{115.5mm}
            \begin{minipage}[b]{114.5mm}
            \raggedright
            \begin{list}{}{\labelwidth9mm
                           \leftmargin9mm
                           \labelsep0mm}
%ho            \item[#1 \hfill] #3 \newline
%ho                        {\em #4}\dotfill
%             \item[#1 \hfill] {\em #2:} #4 #3 \dotfill
            \item[#1 \hfill] #3: #2 \dotfill  % #1 = Buchstabe und lfd. Nr.; #2 = Autoren; #3 = Autoren ;#4 = Titel
            \end{list}
            \end{minipage}
%ho            \begin{minipage}{5.5mm}
            \begin{minipage}{6.5mm}
%             \hfill\raisebox{1.5pt}{\the\tocpos} % Seitennummer
%             \hfill\raisebox{1.5pt} 
	      \hfill \raisebox{1.5pt}{#5}
            \end{minipage}
%             \addauthor{#5}
%             \addpreindex{#7}
%             \addcategory{#6}
%             \advance \tocpos #2\relax % advance erhöht/vermindert die Variable tocpos; relax macht nichts (no-op) = Abbruch ohne Fehlermeldung
%             \advance \tocpos \relax % advance erhöht/vermindert die Variable tocpos; relax macht nichts (no-op) = Abbruch ohne Fehlermeldung
        }


\newcommand{\firma}[1]
           {\begin{minipage}[t]{58mm}
             #1
            \end{minipage}}

\newcommand{\siehe}[2]{#2, {\it siehe} #1}

\newcommand{\nachsatz}[2]{#1, #2}

\newcommand{\nachsatzfett}[2]{#1, {\bf #2}}

\newcommand{\fett}[1]{{\bf #1}}

\newcommand{\fettumbruch}[1]{{\bf #1} \newpage}

\newcommand{\umbruch}[1]{#1 \newpage}

\newcommand{\zwischen}[1]
           {\newpage
            \rule{0mm}{0mm}

            \vspace{5cm}
            \begin{center}
            \baselineskip35pt
            {\huge \bf #1} 
            \end{center}}

%	Pseudo-Definition für tocgenerate
\newcommand{\pagecount}[1]{}


\newcommand{\elqq}{``}%
\newcommand{\erqq}{''}%
